T1: Scaling Diffusion Probabilistic Fields to High-Resolution on Unified Visual Modalities

Diffusion Probabilistic Field (DPF) models the distribution of continuous functions defined over metric spaces. While DPF shows great potential for unifying data generation of various modalities including images, videos, and 3D geometry, it does not scale to a higher data resolution. This can be attributed to the ``scaling property'', where it is difficult for the model to capture local structures through uniform sampling. To this end, we propose a new model comprising of a view-wise sampling algorithm to focus on local structure learning, and incorporating additional guidance, e.g., text description, to complement the global geometry. The model can be scaled to generate high-resolution data while unifying multiple modalities. Experimental results on data generation in various modalities demonstrate the effectiveness of our model, as well as its potential as a foundation framework for scalable modality-unified visual content generation.

==> 3d.tex <==
\begin{figure}[tbp]
    \centering
    \begin{subfigure}{.31\textwidth}
    \includegraphics[width=\textwidth]{neurips_2023/results/shapenet/pixelnerf.png}
    \caption{pixelNeRF~\cite{yu2021pixelnerf}}
    \end{subfigure}
    \hfill
    \begin{subfigure}{.31\textwidth}
    \includegraphics[width=\textwidth]{neurips_2023/results/shapenet/functa.png}
    \caption{Functa~\cite{dupont2022data}}
    \end{subfigure}    
    \hfill
    \begin{subfigure}{.31\textwidth}
    \includegraphics[width=\textwidth]{neurips_2023/results/shapenet/ours.png}
    \caption{\textbf{T1} (Ours)}
    \end{subfigure}
    \hfill

    \begin{subfigure}{\textwidth}
    \includegraphics[width=\textwidth]{neurips_2023/results/shapenet/our_high.png}
    \caption{\textbf{T1} (Our high-resolution result)}
    \end{subfigure}
    \hfill
    
    \caption{Qualitative comparisons of domain-specific novel view synthesis models and ours. Our results show competitive quality without explicitly using 3D modeling and allows generating high-resolution results (\emph{e.g.}, 256$\times$256$\times$251 ) by only using low-resolution training data.}
    \vspace{-1\baselineskip}
    \label{fig:3d}
\end{figure}

==> diffusion_commands.tex <==
\usepackage{amsmath,amsfonts,bm}

\newcommand{\defeq}{\coloneqq}
\newcommand{\grad}{\nabla}
\newcommand{\Ea}[1]{\E\left[#1\right]}
\newcommand{\Eb}[2]{\E_{#1}\!\left[#2\right]}
\newcommand{\Vara}[1]{\Var\left[#1\right]}
\newcommand{\Varb}[2]{\Var_{#1}\left[#2\right]}
\newcommand{\kl}[2]{D_{\mathrm{KL}}\!\left(#1 ~ \| ~ #2\right)}
\newcommand{\bA}{\mathbf{A}}
\newcommand{\bI}{\mathbf{I}}
\newcommand{\bJ}{\mathbf{J}}
\newcommand{\bH}{\mathbf{H}}
\newcommand{\bL}{\mathbf{L}}
\newcommand{\bM}{\mathbf{M}}
\newcommand{\bQ}{\mathbf{Q}}
\newcommand{\bR}{\mathbf{R}}
\newcommand{\bzero}{\mathbf{0}}
\newcommand{\bone}{\mathbf{1}}
\newcommand{\bb}{\mathbf{b}}
\newcommand{\bu}{\mathbf{u}}
\newcommand{\bv}{\mathbf{v}}
\newcommand{\bw}{\mathbf{w}}
\newcommand{\bx}{\mathbf{x}}
\newcommand{\by}{\mathbf{y}}
\newcommand{\bz}{\mathbf{z}}
\newcommand{\bxh}{\hat{\mathbf{x}}}
\newcommand{\btheta}{{\boldsymbol{\theta}}}
\newcommand{\bphi}{{\boldsymbol{\phi}}}
\newcommand{\bepsilon}{{\boldsymbol{\epsilon}}}
\newcommand{\brho}{{\boldsymbol{\rho}}}
\newcommand{\bmu}{{\boldsymbol{\mu}}}
\newcommand{\bnu}{{\boldsymbol{\nu}}}
\newcommand{\bSigma}{{\boldsymbol{\Sigma}}}

==> math_commands.tex <==

\usepackage{amsmath,amsfonts,bm}

\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

\newcommand{\newterm}[1]{{\bf #1}}


\def\figref#1{figure~\ref{#1}}
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
\def\secref#1{section~\ref{#1}}
\def\Secref#1{Section~\ref{#1}}
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
\def\eqref#1{equation~\ref{#1}}
\def\Eqref#1{Equation~\ref{#1}}
\def\plaineqref#1{\ref{#1}}
\def\chapref#1{chapter~\ref{#1}}
\def\Chapref#1{Chapter~\ref{#1}}
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
\def\algref#1{algorithm~\ref{#1}}
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
\def\partref#1{part~\ref{#1}}
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

\newcommand{\pdata}{p_{\rm{data}}}
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} %

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} %

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> rebuttal.tex <==
\newpage
~
\newpage

\appendix

\section{Rebuttal}

To R#1
1. For single frame, our running time (s) of the content, motion, video generation is {0.3, 0.4, 0.7}, and the memory cost (Mb) is {1244, 2499, 3743}. For reference, StyleGAN-V is 0.04s and 3120 Mb but only gets 27.83 FID, while ours is 10.94 FID. Even though autoregressive enlarge the efficiency issue, ours is more scalable than the concurrent VDM using 3D UNet. For training efficiency, our training cost is 4 A6000 GPUs for 6 days, while VDM is trained with 256 TPU-v4 chips.

2. We will update the going user study in revision and would like to refer to the supplemental with many video result comparisons. 

3. Due to space limitations, we will certainly discuss these concurrent work details in revision.

To R#5
1. Specifically, the latent is estimated by a network v(.) that takes the first x(0) and last x(n−1) frame as input for the n-th frame generation. It assumes the last frame can represent the continuous dynamics of the video once the previous frames are correct. Compared with 3D CNN, ours allows more diverse dynamics modeling with more efficient network design. It is also assumed by most advanced video generation methods, including DIGAN (it uses two randomly generated frames ) and StyleGAN-V (it uses two continuous frames). We also have experimented with using v(x(0)), v(x(n−1)), v(x(n−2), x(n−1)), and v(x(0), x(n−1), x(n−2)) but none of they can achieve better results than v(x(0), x(n-1)).

2. Please see our first response to R#1.

To R#6
1. Our primary intuition is to prevent zero values; thus, a relatively small value is selected. Since the original L1 loss is not differentiable at zero values, the zero values will cause the gradient to vanish and leave some parameters unchanged. In contrast, adding a relatively small value ensures non-zero values. We experimentally find that 1e-8 is the best value for CLEVRER, but we suggest the value should be empirically chosen as hyper-parameters. We experimented with values of {1e-5, 1e-6, 1e-7, 1e-8} and got FID results of {19.2, 19.1, 18.7, 18.4}. We will update them in revision to illuminate this.

2. SpyNet is the most fundamental optical flow estimation network architecture and has been demonstrated in motion extraction for video enhancement and interpolation. Inspired by it, we chose its network architecture as our latent encoder v(.) to represent video dynamics, and we empirically found it fits the implicit latent distribution well upon training. Besides, the weights of the pretrained SpyNet substantially serve as the weight initialization scheme of encoder v(.) and can be replaced with slight performance loss. We will update the intuition in revision to clarify. 

3. Residual modeling has been demonstrated in diffusion networks like deblurring (e.g., Deblurring via Stochastic Refinement). We experimentally find that our adaptive feature residual component is crucial in modeling complex scenes of video data (like UCF101). In particular, our adaptive feature residual component achieves a significant 49 FVD improvement in UCF101, while 3 FVD improvement in CLEVER. We will highlight the improvement in our final edition for precise.

4. We sincerely appreciate your suggestion since VDM was the only published diffusion-based video model before the submission. Compared with the concurrent Flexible Diffusion Modeling of Long Videos, ours models video dynamics between two frames as the condition latent. Therefore, our new paradigm better fits the diffusion network and is more scalable for high-resolution video generation. Given the substantial paradigm difference, we believe our contribution is still significant. We will update more comparisons and discussions in revision.

5. Thank you for your suggestion. We have fixed typos thoroughly (e.g., “regards” → “regard” and “implicitly” → “implicit” in page 2) in revision.

To R#7: We sincerely argue that our method is non-trivial because:

- Existing works for video generation would fail at high-resolution, long video data due to its spatio-temporal complexity. We first investigate the relationships between the video dynamics and manifold manipulation effects of conditions, which can model dynamics as the trajectory of content subspace traversing. Thus, we propose an implicit condition mechanism and demonstrate its flexible and scalable properties on high-resolution, long video data.

- Previous works solely depend on the 3D CNN or INRs for modeling continuous video dynamics. The first method requires heavy computation (VDM), while the second cannot apply to diffusion networks (StyleGAN-V). Inspired by the recent feature modulation mechanism for style decomposition, we propose a new fashion by taking positional encoded dynamic features as the normalization statistics. We show that it fits the diffusion network well and avoids heavy computation during modeling.

Our method also contains various novel (yet simple) components. We believe they would greatly inspire the community.

==> sota.tex <==

\begin{table}[t]
    \setlength\tabcolsep{4pt}
    \begin{center}
    \resizebox{\linewidth}{!}{
    \begin{tabular}[t]{rcccccccccc}
    \toprule
    \multirow{2.5}{*}{\bf Model} & \multicolumn{3}{c}{\bf{CelebA-HQ} 64$\times$64} & \multicolumn{3}{c}{\bf{CelebV-Text} 256$\times$256$\times$128} & \multicolumn{4}{c}{\bf{ShapeNet-Cars} 128$\times$128$\times$251}  \\
    \cmidrule(r){2-4} \cmidrule(r){5-7} \cmidrule(r){8-11}
     & FID ($\downarrow$) & Pre. ($\uparrow$) & Rec. ($\uparrow$) & FVD ($\downarrow$) & FID ($\downarrow$) & CLIPSIM ($\uparrow$) & FID ($\downarrow$) & LPIPS ($\downarrow$) & PSNR ($\uparrow$) & SSIM ($\uparrow$) \\
    \midrule
    Functa~\cite{dupont_data_2022} & 40.40 & 0.58 & 0.40 & \xmark & \xmark & \xmark & 80.3 & N/A & N/A & N/A \\
    GEM~\cite{du2021learning} & 30.42 & 0.64 & 0.50 & \xmark & \xmark & \xmark & \xmark & \xmark & \xmark & \xmark  \\
    GASP~\cite{dupont2021generative} & 13.50 & 0.84 & 0.31 & \xmark & \xmark & \xmark & \xmark & \xmark & \xmark & \xmark  \\
    DPF~\cite{zhuang_diffusion_2023} & 13.21 & \textbf{0.87} & 0.35 & \xmark & \xmark & \xmark & \xmark & \xmark & \xmark & \xmark \\
    \midrule
    TFGAN~\cite{balaji2019conditional} & \xmark & \xmark & \xmark & 571.34 & 784.93 & 0.154 & \xmark & \xmark & \xmark & \xmark  \\
    MMVID~\cite{han_show_2022} & \xmark & \xmark & \xmark & 109.25 & 82.55 & 0.174 & \xmark & \xmark & \xmark & \xmark \\
    MMVID-interp~\cite{han_show_2022} & \xmark & \xmark & \xmark & 80.81 & 70.88 & 0.176 & \xmark & \xmark & \xmark & \xmark \\
    VDM~\cite{ho_video_2022} & \xmark & \xmark & \xmark & 81.44 & 90.28 & 0.162 & \xmark & \xmark & \xmark & \xmark \\
    CogVideo~\cite{hong2022cogvideo} & \xmark & \xmark & \xmark & 99.28 & 54.05 & 0.186 & \xmark & \xmark & \xmark & \xmark \\
    \midrule
    EG3D-PTI~\cite{chan2022efficient} & \xmark & \xmark & \xmark & \xmark & \xmark & \xmark & 20.82 & 0.146 & 19.0 & 0.85 \\
    ViewFormer~\cite{kulhanek2022viewformer} & \xmark & \xmark & \xmark & \xmark & \xmark & \xmark & 27.23 & 0.150 & 19.0 & 0.83 \\
    pixelNeRF~\cite{yu2021pixelnerf} & \xmark & \xmark & \xmark & \xmark & \xmark & \xmark & 65.83 & 0.146 & 23.2 & 0.90 \\
    \midrule
    \textbf{T1 (Ours)} & \textbf{5.55} & 0.77 & \textbf{0.51} & \textbf{42.03} & \textbf{24.33} & \textbf{0.220} & 24.36 & \textbf{0.118} & \textbf{23.9} & \textbf{0.90}  \\
    \bottomrule
    \end{tabular}
    }
    \end{center}
    \caption{Sample quality comparison with state-of-the-art models for each task. ``\xmark'' denotes the method cannot be adopted to the modality due to the method design or impractical computation cost.}
    \vspace{-1\baselineskip}
    \label{tab:sota}
\end{table}

==> teaser.tex <==
\begin{figure}[htbp]
    \centering
    \includegraphics[width=.96\textwidth]{example-image-golden}
    \caption{Selected generalized results of our approach adapted to different domains.}
    \label{fig:teaser}
    \vspace{-2\baselineskip}
\end{figure}

==> video_compare.tex <==

\begin{figure}[htbp]
    \centering
    \begin{subfigure}[b]{1\textwidth}
    \centering
    \includegraphics[width=.13\textwidth]{neurips_2023/results/celebv/vdm/vdm001.png}
    \includegraphics[width=.13\textwidth]{neurips_2023/results/celebv/vdm/vdm006.png}
    \includegraphics[width=.13\textwidth]{neurips_2023/results/celebv/vdm/vdm011.png}
    \includegraphics[width=.13\textwidth]{neurips_2023/results/celebv/vdm/vdm016.png}
    \includegraphics[width=.13\textwidth]{neurips_2023/results/celebv/vdm/vdm021.png}
    \includegraphics[width=.13\textwidth]{neurips_2023/results/celebv/vdm/vdm026.png}
    \includegraphics[width=.13\textwidth]{neurips_2023/results/celebv/vdm/vdm031.png}
    \hfill
    \caption{VDM~\cite{ho_video_2022}}
    \end{subfigure}
    
    \begin{subfigure}[b]{1\textwidth}
    \centering
    \includegraphics[width=.13\textwidth]{neurips_2023/results/celebv/cogvideo/2e8ab9a913e1421d9b31ca5d566c5c30RKNTlpYaz8A9TVXE-0.png}
    \includegraphics[width=.13\textwidth]{neurips_2023/results/celebv/cogvideo/2e8ab9a913e1421d9b31ca5d566c5c30RKNTlpYaz8A9TVXE-4.png}
    \includegraphics[width=.13\textwidth]{neurips_2023/results/celebv/cogvideo/2e8ab9a913e1421d9b31ca5d566c5c30RKNTlpYaz8A9TVXE-8.png}
    \includegraphics[width=.13\textwidth]{neurips_2023/results/celebv/cogvideo/2e8ab9a913e1421d9b31ca5d566c5c30RKNTlpYaz8A9TVXE-12.png}
    \includegraphics[width=.13\textwidth]{neurips_2023/results/celebv/cogvideo/2e8ab9a913e1421d9b31ca5d566c5c30RKNTlpYaz8A9TVXE-16.png}
    \includegraphics[width=.13\textwidth]{neurips_2023/results/celebv/cogvideo/2e8ab9a913e1421d9b31ca5d566c5c30RKNTlpYaz8A9TVXE-20.png}
    \includegraphics[width=.13\textwidth]{neurips_2023/results/celebv/cogvideo/2e8ab9a913e1421d9b31ca5d566c5c30RKNTlpYaz8A9TVXE-24.png}
    \hfill
    \caption{CogVideo~\cite{hong2022cogvideo}}
    \end{subfigure}

    \begin{subfigure}[b]{1\textwidth}
    \centering
    \centering
    \includegraphics[width=.13\textwidth]{neurips_2023/results/celebv/ours/0003.png}
    \includegraphics[width=.13\textwidth]{neurips_2023/results/celebv/ours/0005.png}
    \includegraphics[width=.13\textwidth]{neurips_2023/results/celebv/ours/0007.png}
    \includegraphics[width=.13\textwidth]{neurips_2023/results/celebv/ours/0009.png}
    \includegraphics[width=.13\textwidth]{neurips_2023/results/celebv/ours/0011.png}
    \includegraphics[width=.13\textwidth]{neurips_2023/results/celebv/ours/0013.png}
    \includegraphics[width=.13\textwidth]{neurips_2023/results/celebv/ours/0015.png}
    \caption{\textbf{T1} (Ours)}
    \end{subfigure}
    \caption{Qualitative comparisons of domain-specific text-to-video models and ours with prompt: ``\emph{This young female has straight hair. She has long black hair. The woman has arched eyebrows and bags under eyes. She smiles all the time.}'' Compared with VDM~\cite{ho_video_2022}, our result is more continuous. Compared with CogVideo~\cite{hong2022cogvideo}, our result have more realistic textures, \emph{e.g.}, of the hair.}
    \label{fig:video}
\end{figure}

